Improving Screening Processes via Calibrated Subset Selection

Many selection processes such as finding patients qualifying for a medical trial or retrieval pipelines in search engines consist of multiple stages, where an initial screening stage focuses the resources on shortlisting the most promising candidates. In this paper, we investigate what guarantees a screening classifier can provide, independently of whether it is constructed manually or trained. We find that current solutions do not enjoy distribution-free theoretical guarantees -- we show that, in general, even for a perfectly calibrated classifier, there always exist specific pools of candidates for which its shortlist is suboptimal. Then, we develop a distribution-free screening algorithm -- called Calibrated Subset Selection (CSS) -- that, given any classifier and some amount of calibration data, finds near-optimal shortlists of candidates that contain a desired number of qualified candidates in expectation. Moreover, we show that a variant of CSS that calibrates a given classifier multiple times across specific groups can create shortlists with provable diversity guarantees. Experiments on US Census survey data validate our theoretical results and show that the shortlists provided by our algorithm are superior to those provided by several competitive baselines.

==> screening-calibrated-subset-selection (1)/000abstract.tex <==
Many selection processes such as finding patients qualifying for a medical trial or retrieval pipelines in search 
engines consist of multiple stages, where an initial screening stage focuses the resources on shortlisting the most 
promising candidates. 
%
In this paper, we investigate what guarantees a screening classifier can provide, independently of whether it is 
constructed manually or trained. 
%
We find that current solutions do not enjoy distribution-free theoretical guarantees---we show that, in general, 
even for a perfectly calibrated classifier, there always exist specific pools of candidates for which its shortlist 
is suboptimal. 
%
Then, we develop a distribution-free screening algorithm---called \algname (\algabbrNS)---that, given any classifier and some amount of calibration 
data, finds near-optimal shortlists of candidates that contain a desired number of qualified candidates in expectation. 
%
Moreover, we show that a variant of CSS that calibrates a given classifier multiple times across specific 
groups can create shortlists with provable diversity gua\-ran\-tees. 
%
Experiments on US Census survey data validate our theoretical results and show that the shortlists provided by our 
algorithm are superior to those provided by several competitive baselines.


==> screening-calibrated-subset-selection (1)/010introduction.tex <==
Screening is an essential part of many selection processes, where an often intractable number of candidates is reduced to a shortlist of the most promising candidates for detailed---and more resource intensive---evaluation. Screening thus enables an allocation of resources that improves the overall quality of the decisions under limited resources. Examples of such screening problems are: finding patients in a large database of electronic health records to manually evaluate for qualification to take part in a medical trial~\cite{liu2021evaluating}; the first stage of a multi-stage retrieval pipeline of a search engine~\cite{covington2016deep,geyik2019fairness}; or which people to reach out to with a personalized invitation to apply to a specific job posting~\cite{raghavan2020mitigating}.  
In each of these examples, there is significant pressure to make high-qua\-li\-ty, 
unbiased screening decisions quickly and efficiently, often about thousands or even millions 
of candidates under limited re\-sour\-ces and additional diversity requirements~\cite{bendick1997employment,bertrand2004emily,johnson2016if,covington2016deep}.
While these screening decisions have been made manually or through manually constructed rules in the past, automated predictive tools for optimizing screening decisions are becoming more prevalent~\cite{cowgill2018bias, chamorro2019should, raghavan2020mitigating, sanchez2020does}.

Algorithmic screening has been typically studied together with other high-stakes decision making problems as a
supervised learning problem~\cite{corbett2017algorithmic, kilbertus2020fair,sahoo2021reliable}. Under this perspective, algorithmic screening reduces to: 
%
% \begin{itemize}[nolistsep, leftmargin=0.7cm]
%\item[(i)] 
(i) training a classi\-fier that estimates the probability that 
a candidate is \emph{qualified} given a set of observable features;
% conditional -> saving space
%
% \item[(ii)] 
(ii) de\-signing a deterministic threshold rule that shortlists candidates by 
thresholding the candidates'{} pro\-ba\-bi\-li\-ty values estimated by the 
classifier.
%
% \end{itemize}
% the training of / the design of
Here, the classifier and the threshold rule aim to maximize a measure of average accuracy 
and average utility, respectively, possibly subject to diversity constraints.
%
Only very recently, it has been argued that the classifier must also satisfy threshold 
calibration, a specific type of group calibration, to be able to accurately estimate the
average utility of the threshold rule~\cite{sahoo2021reliable}.

Unfortunately, the above screening algorithms do not enjoy dis\-tri\-bu\-tion-free guarantees\footnote{We refer to distribution-free guarantees as finite-sample distribution-free guarantees, since we never have infinite amount of data in practice. } on the quality of the shortlisted candidates. % they provide. % given a pool of candidates. 
%
As a result, they may not always hold their promise of increasing the 
efficiency of a selection process without decreasing the quality of the screening decisions.
%
The results in this paper bridge this gap. 
%
In particular, we focus on developing screening algorithms that, without making any distributional assumptions on the candidates, provide the smallest shortlists of candidates, among those in a given pool, con\-tai\-ning a desired expected number of qualified candidates with high probability.\footnote{If the overall pool of candidates does not contain the desired number of qualified candidates with high probability, the algorithms should also determine that.}

% provably provide -> provide since we already say at the end that it is with high probability. Saving space.

\xhdr{Our Contributions}
%
% Talk about our objective, conditional and unconditional. Talk about negative results 
% for conditional. Talk about our algorithm for unconditional. Talk about the variation 
% of our algorithm that increases diversity across demographic groups. Summarize the 
% findings of the experiments.
%
We first show that, even if a classifier is perfectly calibrated, in general,
%
there always exist\- specific pools of candidates for which the shortlist created 
by a policy that makes decisions based on the probability predictions from the classifier 
will be significantly suboptimal, both in terms of the size and the expected number of 
qualified candidates.
%
Then, we develop a distribution-free screening algorithm---called \algname (\algabbrNS)---that cali\-brates any given 
classifier using calibration data in a way such that the shortlist of candidates 
created by thresholding the candidates'{} probability values estimated by the calibrated 
classifier is near-optimal in terms of expected size, and it
%
provably contains, in expectation across all potential pools of candidates, 
a desired number of qualified candidates with high probability.
%
Moreover, we theoretically characterize how the accuracy of the classifier and the amount of 
calibration data affect the expected size of the shortlists \algabbr provides. 
%
In addition, motivated by the Rooney rule~\cite{collins2007tackling}, which requires that,
when hiring for a given position, at least one candidate from the underrepresented group 
be interviewed, 
%
we demonstrate that a variant of \algabbr that calibrates the given classifier
% diverse shortlist -> shortlist / redundant, we say with provable diversity guarantees; saving space.
multiple times across different groups can be used to create a shortlist with provable 
diversity guarantees---this shortlist contains, in expectation across all potential 
pools of candidates, a desired number of qualified candidates from 
each group with high probability.

Finally, we validate \algabbr on simulated screening processes created using  US Census survey 
data~\cite{ding2021retiring}\footnote{Our code is accessible at \url{ https://github.com/LequnWang/Improve-Screening-via-Calibrated-Subset-Selection.} }.
%
The results show that, compared to several competitive baselines, \algabbr consistently 
selects the shortest shortlists of candidates among those methods that select enough qualified candidates.
%
Moreover, the results also demonstrate that the amount of human effort \algabbr helps reducing---the 
difference in size between the pools of candidates and the shortlists it provides---depends on the accuracy 
of the classifier it relies upon as well as the amount of calibration data. 
%
However, the expected quality of the shortlists---the expected number of qualified candidates 
in the shortlists---never decreases below the user-specified requirement.
%
% as predicted by the theory.

\xhdr{Further Related Work}
%
Our work builds upon prior literature on distribution-free uncertainty quantification, which includes calibration and conformal prediction. 

Calibration~\cite{brier1950verification,dawid1982well,platt1999probabilistic,zadrozny2001obtaining,gneiting2007probabilistic,gupta2020distribution} measures the accuracy of the probability outputs from predictive models. Many notions of calibration have been proposed to measure the accuracy of the probability outputs from a classifier~\cite{platt1999probabilistic,guo2017calibration} or a regression model~\cite{gneiting2007probabilistic,kuleshov2018accurate}. Arguably, the most commonly used notion is marginal (or average) calibration~\cite{gupta2020distribution,zhao2020individual,gneiting2007probabilistic,kuleshov2018accurate} for both classifiers and regression models, which requires the probability outputs be marginally calibrated on the whole population. 
Our definition of perfectly calibrated classifier inherits from the marginal calibration definition for classifiers in prior works~\cite{gupta2020distribution}. We also show how \algabbr produces an approximately calibrated regression model under average calibration definition in regression~\cite{gneiting2007probabilistic,kuleshov2018accurate}. In the other extreme, individual calibration~\cite{zhao2020individual} refers to a classifier that predicts the probability distribution for each example. We refer to classifiers with such properties the omniscient classifiers in this paper. 
Many recent works~\cite{chouldechova2017fair,kleinberg2016inherent,pleiss2017neurips} discuss the relationship between calibration and fairness in binary classification, and show that marginal calibration is incompatible with many fairness definitions in machine learning. Motivated by multicalibration~\cite{hebert2018multicalibration,jung2021moment}, which requires the predictive models be calibrated on multiple groups of candidates, we propose a variant of \algabbr that selects calibrated subsets within each group to ensure diversity in the final selected shortlists. Very recently, some works~\cite{sahoo2021reliable,zhao2021calibrating,straitouri2022provably,wang2022fairness} realize that we can design calibration algorithms (and calibration definitions) well-suited for different downstream tasks to achieve better performance. \algabbr is specifically designed for screening processes so that it provides near-optimal shortlists in terms of the expected size among those having distribution-free guarantees on the expected number of qualified candidates.

Conformal prediction~\cite{vovk1999machine,vovk2005algorithmic,shafer2008tutorial,romano2019conformalized,balasubramanian2014conformal, gupta2020distribution, angelopoulos2021gentle,chzhen2021set} aims to build confidence intervals on the probability outputs from predictive models. Within this literature, the work most closely related to ours is arguably the work by \cite{bates2021distribution}, which 
has focused on generating set-valued predictions from a black-box predictor that controls 
the expected loss on future test points at a user-specified level.
%
While one can view our problem from the perspective of set-valued predictions, applying 
their me\-tho\-do\-lo\-gy to find near-optimal solutions in our problem is not straightforward, and one would need 
to assume to have access to qualification labels for all the candidates in multiple pools, something 
we view as rather impractical. 
%

Moreover, our work also builds on work in budget-constrained decision making, where one needs to first select a
set of candidates to screen and then, given the result of that screening process, determine to whom to allocate
the resources~\cite{cai2020fair, bakker2021beyond}. 
%
This contrasts with our work where all candidates undergo screening. 
%

Many large-scale recommender systems adopt multi-stage pipelines~\cite{bendick2013developing}. Existing works on
multi-stage recommender systems~\cite{ma2020off,hron2021component} focus on learning accurate classifiers in
different stages. Complementary to these works, we assume the classifiers are already given and provide
distribution-free and finite-sample guarantees on the quality of the shortlists. 

==> screening-calibrated-subset-selection (1)/020formulation.tex <==
Given a candidate with a feature vector $x \in \Xcal$, 
we assume the candidate can be either qualified 
($y = 1$) or unqualified ($y = 0$) for the selection objective\footnote{In practice, one needs to measure 
qualification using proxy variables and these proxy variables need to be chosen carefully to not perpetuate 
historical biases~\cite{bogen2018help,garr2019diversity,tambe2019artificial}.}. 
%
Moreover, let $f \,:\, \Xcal \rightarrow [0, 1]$ be a classifier that maps a candidate'{}s feature vector $x$ 
to a quality score\footnote{Our theory and algorithms apply to any classifier with a bounded range, by scaling the scores to $[0,1]$.} $f(x)$. The higher the quality score $f(x)$, the more the classifier believes 
the candidate is qualified. 
%
% Here, without loss of generality\footnote{Our theory and algorithms apply to any classifier with a bounded range, by scaling the scores to $[0,1]$.}, we assume that $\range(f) \subseteq [0, 1]$.
%
% Without loss of generality, we assume that $\Fcal = [0, 1]$.
%
Given a pool of $m$ candidates with feature vectors $\xb~=~\{x_i\}_{i \in [m]}$, 
an algorithmic screening policy \- $\pi \,:\, [0, 1]^{m} \rightarrow \Pcal(\{0, 1\}^{m})$ maps the candidates'{} quality scores 
$\{f(x_i)\}_{i \in [m]}$ to a pro\-ba\-bi\-li\-ty distribution over shortlisting 
decisions $\sbb = \{s_i\}_{i \in [m]}$.
%
Here, each shortlisting decision $s_i$ specifies whether the corresponding candidate is 
shortlisted ($s_i = 1$) or is not shortlisted ($s_i = 0$).
For brevity, we will write $\Sbb \sim \pi$ whenever there is no ambiguity\footnote{We use upper case letters to denote random variables, and lower case letters to denote realizations of random variables.}. 
% for ease of exposition.
%
Furthermore, we use $\pi_f$ to indicate that a policy makes shortlisting decisions based on the quality scores 
from classifier $f$. 
%
% to make the dependence on $f$ more explicit. 
%
% Under $\pi_f$, 
This implies that for any pool of candidates $\xb$ and any two candidates $i,j\in[m]$ in the pool, if $f(x_i)=f(x_j)$, then 
$\Pr(S_i=1) = \Pr(S_j=1)$.
%
We denote the set of all possible policies $\pi_f$ as $\Pi_f$. 
%

For any screening process, we would ideally like a scree\-ning policy $\pi$ that shortlists \emph{only} candidates who are qualified ($y = 1$).
%
Unfortunately, as long as there is no deterministic mapping between $x$ and $y$, such a \emph{perfect} 
screening policy $\pi$ does not exist in general.
%
Instead, our goal is to find a screening policy $\pi$ that shortlists a small set of candidates that provably contains \emph{enough} qualified candidates, without making any assumptions about the data distribution. 
% with high probability
%
These shortlisted candidates will then move forward in the selection process and will be evaluated in detail, possibly multiple times, until one or more qualified candidates are selected. 

More specifically, 
let each candidate'{}s feature vector $x$ and label $y$ be sampled from a data distribution $P_{X,Y} = P_{X} \times P_{Y \given X}$. 
%
Then, for a pool of $m$ candidates\footnote{For ease of presentation, we assume a constant pool size $m$ in 
the main paper. However, all the theoretical results and algorithms can be easily adapted to settings where 
the pool size changes across selection processes. Refer to Appendix~\ref{app:dynamic-pool-size} for more 
details.} with feature vectors $\Xb = \{X_i\}_{i\in[m]}$ and unobserved labels $\Yb = \{Y_i\}_{i\in[m]}$, 
where $X_i \sim P_X$, $Y_i\sim P_{Y\mid X_i}$ for all $i\in[m]$, we will investigate to what extent it is 
possible to find screening policies $\pi$ with near-optimal guarantees with respect to two different oracle 
policies. 
%
In particular: 
%
\begin{itemize}[nolistsep, leftmargin=0.8cm]
\item[(i)] an oracle policy $\pi^{\star}$ that, for any set of candidates $\xb\in\Xcal^m$, shortlists the smallest set of candidates that contains, in expectation with respect to $P_{Y \given X}$, more than $k$ qualified candidates, \ie, $\forall \xb\in\Xcal^m$, 
%
\begin{equation}
    \pi^{\star} \in \argmin_{\pi \in \Pi} \, \EE_{\Sbb \sim \pi}\left[ \sum_{i \in [m]} S_i \right],
    \label{eq:oracle-policy-individual}
\end{equation}
%
where 
%
\begin{equation*}
\Pi = \left\{ \pi \lgiven \EE_{\Sbb \sim \pi, \Yb \sim P} \left[ \sum_{i \in [m]} S_i Y_i \right] \geq k \right\}.
\end{equation*}
% and the shortlisting decisions $\Sbb \sim \pi$. % for all $i \in [m]$.
%
\item[(ii)] an oracle policy $\pi^{\star\star}$ that shortlists the smallest set of candidates that contains, in expectation with respect to $P_{X,Y}$, more than $k$ qualified candidates, \ie, 
%
\begin{equation}
    % \begin{split}
       \pi^{\star\star} \in \argmin_{\pi \in \Pi} \, \EE_{\Xb \sim P, \Sbb \sim \pi} \left[ \sum_{i \in [m]} S_i \right], % \\
       %  \text{subject to} &\quad \EE \left[ \sum_{i \in [m]} S_i Y_i \right] \geq k,
   %  \end{split}
    \label{eq:oracle-policy-marginal}
\end{equation}
%
where 
%
\begin{equation*}
\Pi = \left\{ \pi \lgiven \EE_{(\Xb, \Yb) \sim P, \Sbb \sim \pi} \left[ \sum_{i \in [m]} S_i Y_i \right] \geq k \right\}.
\end{equation*}
%
% and the shortlisting decisions $\Sbb \sim \pi$. % for all $i \in [m]$.
%
\end{itemize}
%
In the language of distribution-free uncertainty quantification~\cite{balasubramanian2014conformal}, the optimality 
guarantees with respect to the first and the second oracle policy can be viewed as individual and marginal guarantees
respectively.
%


==> screening-calibrated-subset-selection (1)/030individual.tex <==
If we had access to an omniscient classifier $f^{\star}(x) = \Pr(Y = 1 \given X = x)$ 
for all $x \in \Xcal$, then we could recover the oracle policy 
$\pi^{\star}$ defined by Eq.~\ref{eq:oracle-policy-individual} just 
by thres\-hol\-ding the quality scores of each candidate in the pool.
%
More specifically, we have the following theorem\footnote{All proofs 
can be found in Appendix~\ref{app:proofs}.}.
%
\begin{theorem} % [Optimal Policy Given Omniscient Classifiers] 
\label{thm:omniscient-classifier-individual}
% Let $f^{\star}(x)$ be the omniscient classifier for a data distribution $P(X, Y)$, \ie, 
% $f^{\star}(x) = P(Y = 1 \given X=x)$ for all $x \in \Xcal$. 
%
The screening policy $\pi^\star_{f^{\star}}$ that, given any pool of $m$ candidates with feature vectors $\xb\in\Xcal^m$,  takes shortlisting decisions as
%
\begin{equation}
\label{eq:decision_rule_omniscient_classifier}
s_i =
\begin{cases}
1 & \textnormal{if} \, f^{\star}(x_i)> t^\star, \\
\textnormal{Bernoulli}(\theta^\star) & \textnormal{if} \, f^{\star}(x_i) = t^\star, \\
0 & \textnormal{otherwise},
\end{cases}
\end{equation}
%
where
\begin{equation*}
t^\star = \sup\left\{t\in[0,1] \lgiven \sum_{i\in[m]}\II\{f^{\star}(x_i)\geq t\}f^{\star}(x_i)\geq k \right\}
\end{equation*}
and
%
\begin{equation*}
    \theta^\star = \frac{k - \sum_{i\in[m]}\II\{f^{\star}(x_i)> t^\star\}f^{\star}(x_i)}{\sum_{i\in[m]}\II\{f^{\star}(x_i)= t^\star\}f^{\star}(x_i)},
\end{equation*}
%
is a solution (if there is one) to the constrained minimization problem  defined in Eq.~\ref{eq:oracle-policy-individual}. 
% manuel: sentence below redundant.
% for any pool of candidates $\xb\in\Xcal^m$. 
\end{theorem}
%
Unfortunately, without distributional assumptions about $P_{X,Y}$, finding the omniscient classifier $f^{\star}$ from 
data is impossible, even asymptotically, if the distribution $P_{f^{\star}(X)}$ induced by $P_{X,Y}$ is nonatomic, as recently shown by Barber~\cite{barber2020distribution} and Gupta et al.~\cite{gupta2020distribution}.
%
Alternatively, one may think whether there exist other classifiers $h$ allowing for near-optimal screening 
policies $\pi_h$ with individual gua\-ran\-tees. 
%
In this context, a natural alternative is a perfectly calibrated classifier $h$ other than the omniscient 
classifier $f^{\star}$. A classifier $h$ is perfectly calibrated if and only if
%
\begin{equation} \label{eq:perfectly-calibrated}
    \Pr(Y=1 \given h(X) = a) = a \quad \forall a\in \range(h).  
\end{equation}
%
However, the following theorem shows that there exist\- data distributions $P_{X,Y}$ for which
there is no perfectly calibrated classifier $h \neq f^{\star}$ allowing for a screening policy $\pi_h$ 
with individual guarantees of optimality.
%
\begin{proposition} \label{prop:impossibility-individual-guarantees}
%
Let $\Xcal = \{ a,b \}$, $\Pr(Y = 1 \given X =a) = 1$, $\Pr(Y = 1 \given X = b) = \frac{k}{m}$,
and $f^{\star}$ be the omniscient classifier.
%
Then, for any screening policy $\pi_h$ using any perfectly calibrated classifier $h \neq f^{\star}$, 
there exists a pool of candidates $\xb=\cbr{x_{i}}_{i\in[m]}\in\Xcal^m$ such that 
%
\begin{equation*}
\left|\EE_{\Sbb \sim \pi_h, \Sbb^{\star} \sim \pi^{\star}_{f^\star}} \left[\sum_{i\in[m]} \left(S_{i} - S^{\star}_{i}\right) \right] \right|\geq \frac{m-k}{2}; 
\end{equation*}
%
% there also exists -> saving space
and a pool of candidates $\xb'=\cbr{x'_{i}}_{i\in[m]}\in\Xcal^m$ such that 
\begin{equation*}
\left|\EE_{\Yb \sim P, \Sbb \sim \pi_h, \Sbb^{\star} \sim \pi^{\star}_{f^\star} } \!\!\!\left[\!\sum_{i\in[m]} \!\!\!\left( S_{i} \!-\! S^{\star}_{i} \right)\! Y_i \right] \!\right|
\geq \frac{k}{2}\!\left(1\!-\!\frac{ k}{m}\right).
\end{equation*}
%\begin{multline*}
%\left|\EE_{\Yb \sim P, \Sbb \sim \pi_h, \Sbb^{\star} \sim \pi^{\star}_{f^\star} } \left[\sum_{i\in[m]} \left( S_{2,i} - S^{\star}_{2,i} \right) Y_i \right] \right| \\
%\geq \frac{k}{2}\left(1-\frac{ k}{m}\right).
%\end{multline*}
%
% where $\Sbb^{\star} \sim \pi^{\star}$ and $\Sbb \sim \pi_h$. 
\end{proposition}
% }
%
The above result reveals that, if $m\gg k$, for any screening policy $\pi_h$ using a calibrated classifier $h \neq f^{\star}$,  there are always scenarios in which $\pi_h$ provides shortlists that are $\frac{m}{2}$ apart from those provided by the oracle policy $\pi^{\star}$ in size or $\frac{k}{2}$ apart in terms of the number of qualified candidates. 
%
In particular, the second part of Proposition~\ref{prop:impossibility-individual-guarantees} directly implies that there is no policy $\pi\in\Pi_h$ that satisfies the individual guarantee. % as stated in the following corollary:
%
% \begin{corollary}
% \label{cor:impossibility-individual-guarantees}
% There exists a data distribution $P_{X,Y}$, such that there is no perfectly calibrated classifier
% $h\neq f^\star$ that is a solution to the optimization problem in 
% Eq.~\ref{eq:oracle-policy-individual} over $\Pi_{h}$ for every $\xb\in\Xcal^m$. 
% \end{corollary}
%
This negative result motivates us to look for screening policies with marginal guarantees of optimality. 
% in the next section. 

==> screening-calibrated-subset-selection (1)/040marginal.tex <==
To investigate to what extent it is possible to find screening policies with near-optimal guarantees with respect to the oracle policy $\pi^{\star\star}$ defined in Eq.~\ref{eq:oracle-policy-marginal}, we focus on perfectly calibrated classifiers $h$ with finite range, \ie, $|\text{Range}(h)| < \infty$.
%
The reason is that, similarly as in the case of the omnis\-cient classifier $f^{\star}$, it is impossible to find nonatomic perfectly calibrated classifiers $h$ from data, even asymptotically~\cite{barber2020distribution,gupta2020distribution}. 
%
We will first introduce the optimal algorithm assuming we have access to a perfectly calibrated classifier, and 
discuss how the accuracy of the classifier affects the performance of the optimal algorithm. 
%
Then, we will introduce the proposed \algabbr algorithm that, given a classifier 
and some amount of calibration data, selects shortlists that are near-optimal in terms of the expected size, while ensuring that the expected number of qualified candidates in the shortlists is above the desired threshold. 

\xhdr{An Optimal Calibration Algorithm with Perfectly Calibrated Classifiers}
%
Let $h$ be a perfectly calibrated classi\-fier with $\text{Range}(h) = \{\mu_b\}_{b\in[B]}$, 
and denote $\rho_b = \EE_{X \sim P}[\II\{h(X) = \mu_b\}]$. % Let $\Pi_h$ be the set of screening policies using classifier $h$.
%
First, note that the classifier $h$ induces a sample-space \emph{partition} of $\Xcal$
into $B$ regions or bins $\{\Xcal_b\}_{b \in [B]}$,
%
where $\mu_b = \Pr(Y = 1 \given X \in \Xcal_b)$ and $\rho_b = \Pr(X \in \Xcal_b)$.
%
Then, the following theorem shows that the optimal screening policy $\pi^{\star}_h$ that shortlists the smallest set of candidates within the set of policies $\Pi_h$, which contain, in expectation with respect to $P_{X,Y}$, more than $k$ qualified candidates, is given by a threshold decision rule.
%
\begin{theorem} \label{thm:perfectly-calibrated-classifier-marginal}
The screening policy $\pi^{\star}_{h}$ that takes shortlisting decisions as
%
\begin{equation*}
s_i =
\begin{cases}
1 & \textnormal{if} \, h(x_i)> t_h, \\
\textnormal{Bernoulli}(\theta_h) & \textnormal{if} \, h(x_i) = t_h, \\
0 & \textnormal{otherwise},
\end{cases}
\end{equation*}
%
where
\begin{equation*}
t_h = \sup\left\{\mu\in \{\mu_b\}_{b\in[B]} \lgiven \sum_{b\in[B]}\mu_{b}\II\{\mu_b\geq \mu\}\rho_b\geq \frac{k}{m}\right\}
\end{equation*}
and
%
\begin{equation*}
    \theta_h = \frac{k/m - \sum_{b\in[B]}\mu_{b}\II\{\mu_b> t_h\}\rho_b}{\sum_{b\in[B]}\mu_{b}\II\{\mu_b=t_h\}\rho_b},
\end{equation*}
%
is a solution (if there is one) to the constrained minimization problem defined in Eq.~\ref{eq:oracle-policy-marginal} over the set of policies $\Pi_h$. 
%
\end{theorem}
%
However, it is important to realize that the expected size of the shortlists provided by 
$\pi^{\star}_h$ for different perfectly calibrated classifiers $h$ may differ. 
%
To put it differently, not all screening policies $\pi^{\star}_h$ (and classifiers $h$) will help reduce the downstream effort by the same amount.
%
To characterize this diffe\-rence, we introduce a notion of dominance between perfectly calibrated classifiers.
%
\begin{definition}
Let $h$ and $h'$ be perfectly calibrated classifiers.
%
We say that $h$ dominates $h'$ if for any $x_1, x_2 \in \Xcal$ such that $h(x_1) = h(x_2)$, it holds that 
$h'(x_1) = h'(x_2)$.
\end{definition}
%
Equipped with this notion, we now characterize the diffe\-rence in size between shortlists provided by different perfectly calibrated classifiers using the following corollary, which follows  
from Theorem~\ref{thm:perfectly-calibrated-classifier-marginal}.
%
\begin{corollary} \label{cor:dominance}
Let $h$ and $h'$ be perfectly calibrated classifiers.
%
If $h$ dominates $h'$, then
%
\begin{equation*}
\EE_{\Xb \sim P, \Sbb \sim \pi^\star_{h}, \Sbb' \sim \pi^\star_{h'}}\left[\sum_{i\in[m]} \rbr{S_i - S'_i} \right] \leq 0. 
\end{equation*}
\end{corollary}
This notion of dominance relates to the notion of sharpness~\cite{gneiting2007probabilistic,kuleshov2018accurate}, which links the accuracy of a calibrated classifier to how fine-grained the calibration is within the sample-space. In particular, if $h$ dominates $h'$, it can be readily shown that $h$ is sharper than $h'$. However, existing works have not studied the effect of the sharpness of a classifier on its performance on screening tasks.
%

\xhdr{A Near-Optimal Screening Algorithm with Calibration Data}
%
Until here, we have assumed that a perfectly calibrated classifier $h$ with finite range, as well as the size 
of each bin $\rho_b$ are given. 
%
However, using finite amounts of calibration data, we can only hope to find \emph{appro\-xi\-ma\-te\-ly} calibrated classifiers.  
% manuel: "and sizes of bins" reads a bit awkward, i think it is ok to skip.
% and sizes of bins.
%
Next, we will develop an algorithm that, rather than training an approximately calibrated classifier from scratch, it \emph{approximately} calibrates a given classi\-fier $f$, \eg, a deep neural network, using a calibration set 
%
$\Dcal_{\text{cal}} = \{ (x_i^c, y_i^c) \}_{i \in [n]}$, 
%
which are independently sampled from $P_{X,Y}$\footnote{Superscript $c$ is used to differentiate between candidates in the calibration set and candidates in the pool at test time.}.
%
% manuel: X_i^{c} -> x_i^{c}, Y_i^{c} -> y_i^{c}. In this context, the calibration data is a set of samples,
% not random variables. The theoretical results are with respect to the randomness of the calibration set,
% which is fine.
%
In doing so, the algorithm will find the optimal sample-space partition and decision rule that minimize the expected size of the provided shortlists among those ensuring that 
an empirical lower bound on the expected number of qualified candidates is greater 
than $k$.

From now on, we will assume that the given classifier $f$ is nonatomic\footnote{We can add arbitrarily small noise to break atoms. } and sa\-tis\-fies a natural 
monotonicity property\footnote{The monotonicity property we consider is different 
from that considered in the literature on monotonic classification~\cite{cano2019monotonic}.} with respect to the data distribution $P_{X,Y}$, a significantly weaker assumption than 
calibration.
%
\begin{definition}
A classifier $f$ is monotone with respect to a data distribution $P_{X,Y}$ if, for any $a, b\in\range(f)$ such that $a<b$, it holds
that
\begin{equation*}
\Pr\cbr{Y = 1 \given f(X) = a} \leq \Pr\cbr{Y = 1 \given f(X) = b}. 
\end{equation*}
\end{definition}
%
Under this assumption\footnote{
% In general, we may unable to test whether a 
% given classifier $f$ is monotone with respect to the data 
% distribution $P_{X,Y}$. 
%
There is empirical evidence that well-performing classifiers learned from data are (approximately) monotone~\cite{guo2017calibration,kuleshov2018accurate,gupta2020distribution}.
%
In this context, we would like to emphasize that the monotone property 
is only necessary to prove that the expected size of the shortlists provided by our algorithm is near-optimal.
%
However, the distribution-free guarantees on the expected number of qualified shortlisted candidates holds even for non-monotone 
classifiers.
%
}, we can first show that 
the solution (if there is one) to the constrained minimization problem in Eq.~\ref{eq:oracle-policy-marginal} over $\Pi_f$ is a threshold decision rule $\pi_{f, t_f^{\star}}$ with some threshold $t_f^{\star}\in[0,1]$ that takes shortlisting decisions as
%
\begin{equation} \label{eq:decision-threshold-rule-algorithm}
s_i =
\begin{cases}
1 & \textnormal{if} \, f(x_i)\geq t_f^{\star}, \\
0 & \textnormal{otherwise}.
\end{cases}
\end{equation}
%
More specifically, we have the following 
theorem.
%
\begin{theorem}
%
\label{thm:optimality_threshold_decision_rules}
Let $f$ be a monotone classifier with respect to $P_{X,Y}$ and the 
distribution $P_{f(X)}$ induced by $P_{X,Y}$ is nonatomic. 
%
Then, for any $\pi_{f} \in \Pi_{f}$, there always exists a threshold decision 
rule $\pi_{f, t} \in \Pi_f$ with some threshold $t\in[0,1]$ such that 
%
\begin{equation*}
\EE_{\Xb\sim P, \Sbb \sim \pi_f, \Sbb' \sim\pi_{f, t}} \left[\sum_{i\in[m]} (S_i - S'_i) \right] \geq 0
\end{equation*}
%
and
%
\begin{equation*}
\EE_{(\Xb, \Yb) \sim P, \Sbb \sim \pi_f, \Sbb' \sim\pi_{f, t}}\left[\sum_{i\in[m]} Y_i (S_i - S'_i)\right] \leq 0. 
\end{equation*}
\end{theorem}
%
The theorem directly implies there exists a threshold decision policy $\pi_{f,t^\star_f}$ that is optimal in the constraint minimization problem in~\ref{eq:oracle-policy-marginal} (if there is a solution). 

% as formally stated in the following corollary. 

% \begin{corollary}
% \label{cor:optimality_threshold_decision_rules}
% Under the same conditions as in Theorem~\ref{thm:optimality_threshold_decision_rules}, there exists a threshold decision policy $\pi_{f,t^\star_f}$ with some threshold $t^\star_f\in[0,1]$ that is a solution (if there is one) to the optimization problem in Eq.~\ref{eq:oracle-policy-marginal}. 
% \end{corollary}

As a result, we focus our attention on finding a near-optimal threshold decision policy. We first notice that each threshold decision policy $\pi_{f,t}$ induces a sample space partition of $\Xcal$ into two bins $\Xcal_{t,1} = \{ x \in \Xcal \given f(x) \geq t \}$ and $\Xcal_{t,2} = \{ x \in \Xcal \given f(x) < t \}$. Thus, it is sufficient to analyze the calibration errors  of the family of approximately calibrated classifiers $h_t$ with the two bins.  
%
In Appendix~\ref{app:screening-multiple-bins}, we show that using the calibration errors of calibrated classifiers that partition the sample-space into more bins will only worsen the performance guarantees of threshold policies. 
%
At this point, one may think of applying conventional dis\-tri\-bu\-tion-free calibration 
methods to bound the calibration errors of each classifier $h_t$ with high probability.
%
However, prior distribution-free calibration methods can only bound calibration errors on the mean values 
$\mu_b$ for each bin $b$, but not the bin sizes $\rho_b$. 
%
To make things worse, to find the threshold value $\hat{t}_f$ with optimal guarantees, we need to bound the 
calibration errors of all classifiers $h_t$, simultaneously with high pro\-ba\-bi\-li\-ty. 
%
Unfortunately, since $t \in [0, 1]$, there are infinitely many of them and we cannot naively apply a union 
bound on the bounds derived separately for each classifier.

To overcome the above issues, we will now leverage the Dvo\-retz\-ky–Kiefer–Wolfowitz–Massart (DKWM) inequality~\cite{dvoretzky1956asymptotic, massart1990tight}, 
which bounds how close an empirical cumulative distribution function (CDF) is to the cumulative distribution function of the distribution from which the empirical samples 
are sampled.
%
More specifically, let $\delta_{t, 1} := \EE_{(X,Y)\sim P}[\II\left\{f(X)\geq t\right\} Y]$ and 
%
\begin{equation*}
    \hat{\delta}_{t, 1} = \frac{1}{n} \sum_{i \in [n]} \II\left\{f(x_i^c)\geq t\right\} y^c_i
\end{equation*}
%
% X_i^{c}, Y^{c}_i -> x_i^{c}, y^{c}_i / in this context, they are samples. This change is consistent
% with the change in line 225 now.
%
be an empirical estimator of $\delta_{t,1}$ using samples from the calibration set $\Dcal_{\text{cal}}$. 
%
Then, we can use the DKWM inequality to bound the calibration errors $|\hat{\delta}_{t, 1}-\delta_{t, 1}|$ across all approximately calibrated classifiers $h_t$ with high probability:
%
\begin{proposition}
\label{prop:bounds_errors_calibration}
For any $\alpha\in (0,1)$, with probability at least $1-\alpha$ (in $f$ and $\Dcal_{\textnormal{cal}}$), it holds that
\begin{equation*}
\left|\delta_{t,1}-\hat{\delta}_{t,1}\right|\leq\sqrt{\ln\left(2/\alpha\right)/(2n)}\coloneqq\epsilon(\alpha,n)  
\end{equation*}
%
simultaneously for all $t \in [0,1]$.
\end{proposition}
%
\begin{algorithm}[t]
\begin{algorithmic}[1]
\STATE{{\bf input:} $k$, $m$, $\Dcal_{\textnormal{cal}}$, $f$, $\alpha$, $\xb$}
\STATE{{\bf initialize:} $\sbb=\mathbf{0}$ }
\STATE{$\hat{t}_f=\sup\cbr{t\in[0,1]\lgiven \hat{\delta}_{t,1} \geq k/m + \epsilon(\alpha,n)}$}
\FOR{ $i=1,\dots,m$ }
\IF{$f(x_i)\geq \hat{t}_f$}
\STATE $s_i = 1$
\ENDIF
\ENDFOR
\STATE{{\bf return} $\sbb$}
\end{algorithmic}
\caption{\algname (\algabbrNS)}
\label{alg:screening}
\end{algorithm}
%
In Appendix~\ref{app:error-bounds-regression-calibration}, we show that based on the above error guarantees, we can build a regression model that achieves average calibration in regression~\cite{gneiting2007probabilistic,kuleshov2018accurate}, if we regard the binary classification problem as a regression problem. 
%
Further, building on the above proposition, we can derive an em\-pi\-ri\-cal lower bound on the expected number of qualified candidates in the shortlists provided by all the threshold decision rules $\pi_{f, t}$.
%
\begin{corollary} \label{cor:bounds_on_objectives}
For any $\alpha\in(0,1)$, with probability at least $1-\alpha$ (in $f$ and $\Dcal_{\textnormal{cal}}$), it holds that 
%
\begin{equation*}
% m\rbr{\hat{\delta}_{t,1} - \epsilon(\alpha,n)}\leq
\EE_{(\Xb,\Yb) \sim P, \Sbb\sim\pi_{f,t}}\left[\sum_{i\in[m]}Y_iS_i\right]
\geq m\rbr{\hat{\delta}_{t,1} - \epsilon(\alpha,n)} 
\end{equation*}
simultaneously for all $t \in [0,1]$.
\end{corollary}
%
Now, to find the decision threshold rule $\pi_{f, \hat{t}_f}$ that provides, in expectation, 
the smallest shortlists of candidates subject to a constraint on the lower bound on 
the expected number of qualified candidates in the provided shortlists, \ie,
%
\begin{equation} \label{eq:optimization_problem_calibration_from_data}
\hat{t}_f = \argmin_{t \in \Tcal} \, \EE_{\Xb\sim P, \Sbb\sim \pi_{f,t}}\left[\sum_{i\in[m]}S_i\right]
\end{equation}
where $\Tcal = \{ t\in[0,1] \given m\rbr{\hat{\delta}_{t,1} - \epsilon(\alpha,n)}\geq k \}$,
%
we resort to the following theorem.
%
\begin{theorem}
\label{thm:calibration_from_data_threshold}
The threshold value
%
\begin{equation}
\label{eq:calibration_from_data_threshold}
\begin{split}
\hat{t}_f = \sup\bigg\{t\in[0,1]\lgiven&\hat{\delta}_{t,1} \geq k/m + \epsilon(\alpha,n)\bigg\} 
\end{split}
\end{equation}
%
is a solution (if there is one) to the constrained minimization problem defined in Eq.~\ref{eq:optimization_problem_calibration_from_data}.
%
\end{theorem}
%
Algorithm~\ref{alg:screening} summarizes our resulting \algabbr algorithm, whose complexity
is $\Ocal(n\log (n))$. %\manuel{Please, luke add the complexity}. 

Finally, we can show that the expected size of the shortlists provided by \algabbr is near-optimal and we can also derive a lower bound on the worst-case size of the provided shortlists.
%
More specifically, the following propositions show that the difference in expected number of qualified
candidates between the shortlists provided by $\pi_{f, \hat{t}_f}$ and $\pi_{f, t^{\star}_f}$ decreases 
at a rate $1/\sqrt{n}$ and the worst-case size is on the order of $\sqrt{k}$.
%
\begin{proposition}
\label{prop:gap_calibration_from_data}
Let $f$ be a monotone classifier with respect to $P_{X,Y}$ and assume that the distribution $P_{f(X)}$ induced by $P_{X,Y}$ is nonatomic. Then, for any $\alpha\in(0,1)$, with probability at least $1-\alpha$, it holds that
\begin{equation*}
    \EE_{(\Xb,\Yb)\sim P, \Sbb \sim \pi_{f, t_f^{\star}}, \Sbb' \sim\pi_{f,\hat{t}_f}}\left[\sum_{i\in[m]} (S'_i - S_i) Y_i\right]
    \leq \frac{m}{n} + m\sqrt{2\ln(2/\alpha)/n}. 
\end{equation*}
\end{proposition}
% Second, not only can Algorithm~\ref{alg:screening} provide guarantees on the expected size of the shortlists, it can 
% also provide a lower bound on the worst-case size of the shortlists. 
\begin{proposition}
\label{prop:PAC_individual_guarantee}
For any $\alpha_1 \in(0,1),\alpha_2\in(e^{-\frac{9}{4}k},1)$ such that $\alpha_1 + \alpha_2<1$, \algabbr with parameter $\alpha = \alpha_1$ guarantees that, with probability at least $1-\alpha_1-\alpha_2$ (in $f$, $\Dcal_{\textnormal{cal}}$, and $\Xb,\Yb$), 
\begin{equation*}
\label{eq:worst-case-guarantee}
\sum_{i\in[m]}\!\!Y_iS_i\geq k - \frac{1}{3}\ln(1\!/\!\alpha_2)
- \frac{1}{3}\sqrt{\ln^2(1\!/\!\alpha_2) \!+\! 18 k\ln(1\!/\!\alpha_2)}. 
\end{equation*}
%\begin{multline}
%\label{eq:worst-case-guarantee}
%\sum_{i\in[m]}Y_iS_i\geq k - \frac{1}{3}\ln(1/\alpha_2) \\
%- \frac{1}{3}\sqrt{\ln^2(1/\alpha_2) + 18 k\ln(1/\alpha_2)}. 
%\end{multline}
\end{proposition}
%
Finally, note that we can use the above worse-case guarantee to ensure that the worst-case size of the shortlists 
provided by \algabbr is greater than a target $t_{\textnormal{worst}}$ by setting $k$ to be 
slightly larger than $k_{\textnormal{worst}}$
%
\begin{equation*}
k = k_{\textnormal{worst}} + \frac{1}{3}\ln(1/\alpha_2) - \frac{1}{3}\sqrt{\ln^2(1/\alpha_2) + 18 k\ln(1/\alpha_2)}. 
\end{equation*}
%
% so that the guarantee on the worst-case shortlist size is greater than the target $t_{\textnormal{worst}}$. 
%
By doing so, \algabbr will satisfy the constraints defined in Eq.~\ref{eq:oracle-policy-individual} 
with high probability with respect to the test pool of candidates.
%
% Algorithm~\ref{alg:screening} satisfies most of the constraints in the individual guarantee 
% as defined in Eq.~\ref{eq:oracle-policy-individual}. 
%
However, \algabbr might not be optimal in terms of expected or worst-case shortlist size among those satisfying 
the above constrains.  
%  that can similarly guarantee enough qualified candidates in the worst case. 
%
How to design screening algorithms that are optimal in terms of expected or worst-case shortlist size while sa\-tisfying
that each individual shortlist contains enough qualified candidates with high probability is an interesting problem 
to explore in future work. 


==> screening-calibrated-subset-selection (1)/050diversity.tex <==
\begin{figure*}[t]
%\vspace{-2mm}
\centering
\includegraphics[width=1.\textwidth]{plots/exp_normal.pdf}
% \vspace{-8mm}
\caption{Analysis of \algabbr and baselines 
when varying the classifier noise ratio $r_{\text{noise}}$ (\ie, accuracy) and calibration
set sizes $n$.
%
The first and third plots show the empirical probability that each algorithm provides enough qualified candidates (EQ) %$EQ=\II\cbr{\hat{\EE}\sbr{\sum_{i\in[m]}Y_iS_i}\geq k}$ 
from $100$ runs with standard error bars (higher is better). 
%
The second and fourth plots show the average, among $100$ runs with one standard deviation as shaded regions, expected size (SS) 
%$SS=\hat{\EE}\sbr{\sum_{i\in[m]}S_i}$ 
of the shortlists (lower is better). We do not plot SS for algorithms that fail the quality requirement in terms of EQ.
%without distribution-free guarantees, since they do not satisfy the constraint to provide enough qualified candidates. 
%
In the left two plots, the size of the calibration set is $n = 10,000$. In the right two plots, the classifier noise ratio
is $r_{\textnormal{noise}} = 0$.
%
}
\label{fig:exp_normal}
% \vspace{-2mm}
\end{figure*}
%
Our theoretical results have shown that \algabbr is robust to the accuracy of the classifier and the amount of calibration data.
%
% in ensuring enough qualified candidates in the shortlists. 
%
However, \algabbr does not account for the potential differences in accuracy or in the amount of calibration data across demographic groups.
%
As a result, qualified candidates in minority groups may be unfairly underrepresented in the shortlists provided by \algabbrNS.
%
% Whenever the classifier is inaccurate or the amount of calibration data
% is small, Algorithm~\ref{alg:screening} provides shortlists with a large
% number of candidates to guarantee that there are enough qualified 
% candidates, as suggested by Corollary~\ref{cor:dominance} and 
% Theorem~\ref{eq:decision-threshold-rule-algorithm}. 

% the macros were introducing a space before ",". I changed to CSS and CSS (Diversity) here.
To tackle the above problem and increase the diversity of the shortlists, we design a variant of \algabbrNS, which we name \algdivabbrNS, motivated by the Rooney rule~\cite{collins2007tackling} and multicalibration~\cite{hebert2018multicalibration} (refer to Appendix~\ref{app:screening-diversity}). 
%
\algdivabbr quantifies the uncertainty
in the estimation of the number of qualified candidates separately for
each demographic group, so that we have distribution-free guarantees for each demographic group. This means that \algdivabbr will include more candidates in the shortlist for groups with higher uncertainty to ensure a sufficient number of qualified candidates from each group.
%
Effectively, \algdivabbr shifts the cost of uncertainty from minority candidates to the decision maker, since it creates a potentially longer shortlist.
%
Interestingly, this provides an economic incentive for the decision maker to both build classifiers that perform well across demographic groups and to collect more calibration data about minority groups. 

==> screening-calibrated-subset-selection (1)/060exp.tex <==
%
% \begin{figure*}[t]
% \centering
% \subfloat[Quality of the shortlists vs. $r_{\text{ratio}}$]{
%     \includegraphics[width=0.235\textwidth]{plots/exp_noise_constraint_satisfied.jpeg}
%     \includegraphics[width=0.235\textwidth]{plots/exp_noise_num_selected.jpeg}
%     \label{fig:exp_quality}
% } \hspace{2mm}
% \subfloat[Quality  of the shortlists vs. $n$]{
%     \includegraphics[width=0.235\textwidth]{plots/exp_cal_size_constraint_satisfied.jpeg}
%     \includegraphics[width=0.235\textwidth]{plots/exp_cal_size_num_selected.jpeg}
%     \label{fig:exp_cal_size}
% }
% \vspace{-1mm}
% \caption{Quality of the shortlists provided by Algorithm~\ref{alg:screening} and several baselines 
% under different values of the classifier noise ratio $r_{\text{ratio}}$ (\ie, accuracy) and calibration
% set sizes $n$.
% %
% In each panel, the left figure shows the expected size of the shortlists each algorithm provide and 
% the right figure shows the percentage of times the shortlists contain at least $k$ number of 
% candidates. 
% %
% In panel (a), the size of the calibration set is $n = 10,000$ and, in panel (b), the classifier noise ratio
% is $r_{\textnormal{noise}} = 0$.
% %
% Shaded regions correspond to one standard deviation.
% }
% \end{figure*}
%

In this section, we compare \algabbr against several competitive baselines on multiple 
instan\-ces of a simulated screening process created using US Census survey data. 
% \footnote{To facilitate research in this area, we will release the code for the the empirical evaluation with the final version of the
% paper. We have submitted an anonymous version of the code with the supplementary material.}
%
% manuel: we already provide the citation below. Saving space.
% ~\cite{ding2021retiring}.
%
% manuel: we say this in the intro and in the abstract, so no need to tell again here.
% saving space
% We find that, in comparison to several competitive baselines, the shortlists provided by 
% \algabbr are consistently the shortest among the methods that select enough qualified candidates
%
% manuel: I would say it is not necessary to summarize everything here.
% Moreover, we also investigate the level of robustness of our algorithm and the baselines 
% with respect to the accuracy of the classifier they rely upon and the amount of calibration 
% data as well as their ability to promote diversity
%, and will be publicly available. 
%

\xhdr{Experiment Setup}
%
We create a simulated screening process using a dataset comprised of employment 
information for $\sim$$3.2$ million individuals from the US Census~\cite{ding2021retiring}. 
%
% The employment prediction task contains the employment information of around $3.2$ million 
% individuals across all the states in the United States. 
%
For each individual, we have sixteen features $x \in \RR^{16}$ (\eg, education, marital 
status) and a label $y\in\{0, 1\}$ that indicates whether the individual is
employed ($y = 1$) or unemployed ($y=0$). 
%
Race is among the features, which we use as the protected attribute as suggested by Ding et al.~\cite{ding2021retiring}. We treat white as the majority group $g_{\textnormal{maj}}$ and all other 
races as the mi\-no\-ri\-ty group $g_{\textnormal{min}}$. 
%
To ensure that there is a limited number of qualified candidates ($\sim$$20$\%) 
in each of the simulated screening processes, we randomly downsample the 
dataset\footnote{For the diversity experiments, we downsample the majority 
and minority groups independently.}.
% , resulting in around $1.67$ million individuals from the majority group and $0.54$ million 
% % individuals from the minority group.}.
%
After downsampling, the dataset contains $\sim$$2.2$ million individuals. 
%

For the experiments, we randomly split the dataset into two equally-sized and disjoint subsets. 
%
% These individuals serve as the data distribution $P_{X,Y}$. 
%
We use one of the subsets to create a training set of $10{,}000$ individuals, as well as calibration sets with varying sizes $n$. We use the other subset to simulate pools of candidates for testing. 
% and the rest $50\%$ of them to sample test lists of candidates. 
%
%, and the data-split process similarly. 
%
To get a screening classifier, we train a logistic regression $f_{\textnormal{LR}}$ on the training set to 
predict the probability $f_{\textnormal{LR}}(x)$ that a candidate is qualified. 
%
Here, we % artificially 
vary the accuracy of the classifier by replacing, with probability $r_{\textnormal{noise}}$, each of its predictions with some noise $\beta\sim\textnormal{Beta}(1, 4)$, \ie, $f=\gamma\beta + (1-\gamma)f_{\textnormal{LR}}$, where $\gamma\sim\textnormal{Bernoulli}(r_{\textnormal{noise}})$ and $r_{\textnormal{noise}}$ is the \emph{classifier~noise~ratio}. 

In each simulated screening process, we set the size of the test pool of candidates to $m = 100$, 
the desired expected number of qualified candidates to $k = 5$,
%
and the success probability to $1 - \alpha = 0.9$.
%
For the diversity experiments, 
% manuel: I think the sentence below is not necessary, if you just sample 100 candidates
% from the downsampled dataset as explained below, they will satisfy what you write below
%
% to test the algorithms that select shortlists from each group independently, we set the number of 
% candidates $m_{\textnormal{maj}}$ and $m_{\textnormal{min}}$ as the expected number of candidates % from each group if we sample $m=100$ candidates (calculated from all the data), and 
%
we set the desired expected number of qualified candidates $k_{\textnormal{maj}}$ and $k_{\textnormal{min}}$ so that the equal opportunity constraint,\ie, $k_{\textnormal{maj}} / (m\EE_{(X,Y)}\sbr{Y\II\cbr{X\in g_{\textnormal{maj}}}}) = k_{\textnormal{min}} / (m\EE_{(X,Y}\sbr{Y\II\cbr{X\in g_{\textnormal{min}}}})$
is satisfied~\cite{hardt2016equality} subject to $k_{\textnormal{maj}} +k_{\textnormal{min}} = 5$.
% and $k_{\textnormal{maj}} +k_{\textnormal{min}} = 5 $ (also calculated from all the data). 
% 
% manuel: we include the info below above now.
% We set the failure probability $\alpha=0.1$ for all experiments. 
%
% manuel: we include the info below above now.
% We randomly sample $n$ individuals as the calibration data, where $n$ varies across experiments 
% and will be specified when we discuss them. 
%
\begin{figure*}[t]
%\vspace{-2mm}
\centering
\includegraphics[width=1.\textwidth]{plots/exp_diversity.pdf}
% \vspace{-5mm}
\caption{Analysis of diversity guarantees of \algdivabbr and several baselines when varying the classifier noise ratio $r_{\text{noise}}$ (\ie, accuracy) for individuals in the minority group.
%
For individuals in the majority group, the classifier noise ratio is $r_{\text{noise}} = 0$.
%
The first and third plots focus on the majority group and the second and fourth plots focus on the minority group.
}
% \vspace{-2mm}
\label{fig:exp_diversity}
\end{figure*}

\xhdr{Methods} In our experiments, we compare \algabbr with several 
baselines. % with and without distribution-free guarantees.
Since no prior screening algorithms with distribution-free guarantees exist, we introduce 
a simple screening algorithm based on uniform mass binning~\cite{zadrozny2001obtaining} (UMB $B$ Bins), which also enjoys distribution-free guarantees on the expected number of qualified candidates. 
%
The algorithm bounds the calibration error of a classifier that is calibrated on $B$ bins of 
roughly equal size and selects the candidates from top-scored bins to low-scored bins (and possibly at random from the last bin it selects candidates from) until a lower bound on the expected 
number of qualified candidates is no smaller than $k$. 
%
Refer to Appendix~\ref{app:screening-multiple-bins} for more details about this baseline algorithm.

We also compare \algabbr with three other baselines that do not provide distribution-free guarantees.
%
The first is called {\em Uncalibrated}, and it applies the optimal decision rule for omniscient classifiers as if $f$ were the omniscient classifier defined in Eq.~\ref{eq:decision_rule_omniscient_classifier}.
%
The second is called {\em Platt}, since it first calibrates $f$ using Platt 
scaling~\cite{platt1999probabilistic} and then proceeds like Uncalibrated with the calibrated classifier.
%
The third is called {\em Isotonic}. It treats the classifier $f$ as a 
regression model from $x$ to $y$, and then employs Isotonic regression calibration~\cite{kuleshov2018accurate} to produce a calibrated regression model $h$ that estimates $h(t)\approx\EE\sbr{(Y\II\cbr{f(x)\geq t}}$. It then selects the largest threshold $t$ such that $mh(t)\geq k$ for shortlisting.

\xhdr{Metrics} To compare the screening algorithms, we run the experiments $100$ times for each algorithm and setting. For each run, we estimate whether each algorithm provides shortlists that contain a large enough expected number of qualified candidates $\textnormal{EQ} = \II\cbr{\hat{\EE}\sbr{\sum_{i\in[m]}Y_iS_i} \geq k}$, and its expected shortlist size $\textnormal{SS} = \hat{\EE}\sbr{\sum_{i\in[m]}S_i}$, using $1,000$ independent pools of candidates sampled at random from the test set. We then compare the algorithms in terms of the percentage of times, along with standard errors, they provide enough qualified candidates. We also compare the average shortlist size, along with standard deviations. 

% For each experiment, we compare the above algorithms in terms of the average size of the shortlists they provide as well as the percentage times the provided shortlists contain at least $k$ qualified candidates in expectation, estimated using $1{,}000$ independent pools of candidates sampled at random from the test set, where,
% for each pool, we sample the candidates'{} labels $1{,}000$ times.

% To calculate the expected size of the shortlist and the expected number of qualified candidates of
% the shortlist, we test the algorithms with $1,000$ randomly sampled test lists of candidates to 
% estimate the expectations. 
%
% For each experiment setting, we run $1,000$ times of the experiments. And for each algorithm, we 
% present the percentage of times ($\pm$ standard error) that it satisfies the constraint in 
% Eq.~\ref{eq:oracle-policy-marginal}, and the expected size of the selected shortlists (mean $\pm$ 
% standard deviation). 
%
% \begin{figure*}[!tbh]
% \begin{subfigure}{.24\textwidth}
%   \centering
%  \includegraphics[width=\linewidth]{plots/exp_diversity_cal_size_constraint_satisfied_maj.jpeg}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{plots/exp_diversity_cal_size_constraint_satisfied_min.jpeg}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%  \centering
%  \includegraphics[width=\linewidth]{plots/exp_diversity_cal_size_num_selected_maj.jpeg}
%\end{subfigure}
%\begin{subfigure}{.24\textwidth}
%  \centering
%  \includegraphics[width=\textwidth]{plots/exp_diversity_cal_size_num_selected_min.jpeg}
%\end{subfigure}
% \vspace*{-0.7\baselineskip}
%\caption{The performance of different algorithms across different groups as we vary the amount of 
%calibration data from the minority group. }
% \vspace*{-1.4\baselineskip}
%\label{fig:exp_diversity_cal_size}
% \end{figure*}
%

% \xhdr{Results}
%
% To structure the exposition of the results, we organize them under the following three research 
% questions.
%

%\noindent \hspace{0mm} --- 
\vspace{1mm} \noindent {\bf How does the accuracy of the classifier affect different screening algorithms?}
% 
% manuel: i added the info below to the caption of the figure, here it is irrelevant for the insights.
% Fixing the number of calibration data at $n = 10,000$, 
%
The left two plots in Figure~\ref{fig:exp_normal} show
how \algabbr compares to the baselines for classifiers of
varying accuracy (\ie, varying $r_{\textnormal{noise}}$). 
%
The results show that the shortlists provided by the algorithms with distribution-free guarantees (i.e., \algabbr and UMB) do contain enough qualified candidates, while the others fail. 
%
% In contrast, all the algorithms with distribution-free guarantees consistently ensure enough 
% qualified candidates in the shortlists across classifiers of different accuracy. 
%
Moreover, \algabbr and UMB are robust to the accuracy of the 
classifier they use, as they compensate for decreased accuracy with longer shortlists to maintain their guarantees.
%---the shortlists they provide are larger as the classifier worsens to guarantee enough qualified candidates are shortlisted. 
%
% This confirms the robustness of the algorithms with distribution-free guarantees to the 
% accuracy of a given classifier, and 
In addition, we find that the shortlists provided by these algorithms contain enough qualified candidates more frequently than suggested by the worst-case theoretical guarantee of $1-\alpha=0.9$. Compared to all UMB variants, \algabbr provides  smaller shortlists except for the pure-noise case.
%, with the exception when the classifier noise ratio is $1$, where UMB $1$ Bin is slightly better.  
%
% since using all the data for calibration gives us smaller calibration error than using only top-scored data when they get top scores only by chance. 
%
Note that this exception does not violate the optimality of \algabbr among deterministic threshold policies using the empirical lower bound as shown in Theorem~\ref{eq:decision-threshold-rule-algorithm}, since UMB algorithms are allowed to randomly select candidates in the last bin they select candidates from, as discussed
previously and in Appendix~\ref{app:screening-multiple-bins} in detail. 
%

%\noindent \hspace{0mm} --- 
\vspace{1mm} \noindent {\bf What is the effect of different amounts of calibration data on the screening algorithms?}
%
% manuel: i added the info below to the caption of the figure, here it is irrelevant for the insights.
% We set the classifier noise ratio at $r_{\textnormal{noise}} = 0$, and 
%
The right two plots in Figure~\ref{fig:exp_normal} show how the screening algorithms perform for increasing amounts of calibration data $n$.
%
We see that \algabbr and UMB are robust to the amount of calibration data, and can effectively account for less data by increasing the shortlist size to maintain their guarantees. In terms of shortlist size, \algabbr is more effective over the whole range of $n$, since it provides smaller shortlists than all of the UMB variants.

%Similarly as before, the results show that the shortlists provided by the algorithms with (without) dis\-tri\-bu\-tion-free guarantees do (not) contain enough qualified candidates.
% algorithms without distribution-free guarantees in general do not ensure enough qualified 
% candidates in the shortlists, while all the algorithms with distribution-free guarantees 
% consistently ensure enough qualified candidates. 
%
%Moreover, the algorithms with distribution-free guarantees are robust to the amount of calibration data---the shortlists they provide are shorter as the amount of calibration data increases and the calibration error is smaller---and, among them, \algabbr provides the smallest shortlists. 

%\noindent \hspace{0mm} --- 
\vspace{1mm} \noindent {\bf How does the accuracy of the classifier affect different groups of candidates?}
%
Figure~\ref{fig:exp_diversity} shows how \algdivabbr and the baselines perform on the majority and minority
groups as we decrease the accuracy of the classifier for individuals in the minority group 
(\ie, we increase $r_{\textnormal{noise}}$ only for individuals in the minority group). 
%
% manuel: i added the info below to the caption of the figure, here it is irrelevant for the insights.
% where we fix the number of calibration data at $n=10,000$. 
%
Here, \algabbr (No Diversity) refers to naively applying \algabbr
on the entire pool of candidates, without diversity requirements. 
%
We allow all other algorithms to select candidates from the majority group and the minority 
group separately. 
%
The results show that, as the accuracy of the classifier for individuals in the minority group decreases, the shortlists provided by \algabbr (No Diversity) contain more and more (fewer and fewer) candidates from the majority (minority) group. 
%
This suggests that we should explicitly account for diversity in the screening process, especially when the accuracy of the classifier differs across groups. 
%
While Uncalibrated, Platt and Isotonic select candidates across groups separately, the
shortlists they provide contain fewer qualified candidates from the minority group as 
the accuracy worsens (Uncalibrated) or do not contain enough qualified candidates from 
both groups (Platt, Isotonic).
%
In contrast, \algdivabbr adapts to the loss in accuracy of the classifier for individuals 
in the minority group and the shortlists it provides contain enough qualified candidates 
from both groups.
%
We found similar results also when we varied the number of individuals from each group in 
the calibration data, instead of the classifier accuracy.
%
%
%
% \begin{figure*}[t]
% \centering
% \subfloat[Qualified candidates in the shortlists]{
%   \includegraphics[width=0.235\textwidth]{plots/exp_diversity_noise_constraint_satisfied_maj.jpeg}
%   \includegraphics[width=0.235\textwidth]{plots/exp_diversity_noise_constraint_satisfied_min.jpeg}
% } \hspace{2mm}
% \subfloat[Number of candidates in the shortlists]{
%   \includegraphics[width=0.235\textwidth]{plots/exp_diversity_noise_num_selected_maj.jpeg}
%   \includegraphics[width=0.235\textwidth]{plots/exp_diversity_noise_num_selected_min.jpeg}
% }
% % \vspace*{-0.7\baselineskip}
% \caption{Quality of the shortlists provided by Algorithm~\ref{alg:screening} and several baselines
% with diversity constraints under different values of the classifier noise ratio $r_{\text{ratio}}$ 
% (\ie, accuracy) for individuals in the minority group.
% %
% For individuals in the majority group, the classifier noise ratio $r_{\text{ratio}} = 0$.
% %
% In each panel, the left figure focus on the majority group and the right figure on the minority
% group.
% }
% \label{fig:exp_diversity_quality}
% \end{figure*}

% \noindent \hspace{0mm} --- \emph{What is the effect of the size of calibration data on different groups 
% of candidates?}
%
% We vary the size $n_{\textnormal{min}}$ of calibration data from the minority group, while fixing the 
% number of calibration data from the majority group at $n_{\textnormal{maj}}$ without any classifier noise
% $r_{\textnormal{noise}}=0$, and plot the performance of different algorithms in 
% \autoref{fig:exp_diversity_cal_size}. We can see that the effect of the size of the calibration data is 
% similar to that of the accuracy of the classifier. Algorithm~\ref{alg:screening} consistently ensures 
% enough qualified candidates, and adapts to the size of the calibration data. All the other algorithms in 
% general fail to ensure enough qualified candidates in the shortlists neither for the majority group nor 
% for the minority group. 

==> screening-calibrated-subset-selection (1)/070conclusions.tex <==
In this work, we initiated the development of screening algorithms that provide distribution-free guarantees on the quality of the shortlisted candidates. 
%
In particular, we proposed the \algabbr algorithm, which can be applied to any screening classifier. We show that for any amount of calibration data, \algabbr selects near-optimal shortlists of candidates, in terms of the expected shortlist size, while ensuring that the expected number of qualified candidates is above a desired target with high probability. Moreover, we showed how the \algdivabbr variant, which shortlists different groups of candidates separately, can ensure diversity of the shortlists with similar guarantees. Both the theoretical analysis and the empirical evaluation confirm that \algabbr and \algdivabbr are robust to the accuracy of the given classifier and the amount of calibration data. 

%
Our work opens up many interesting avenues for future work. 
%
For example,
%
we have assumed that candidates do not present themselves strategically to the screening algorithms
and that the data distribution at calibration and test time is the same.
%
It would thus be interesting to develop screening algorithms that are robust to strategic behaviors~\cite{tsirtsis2020decisions} and distribution shifts~\cite{podkopaev2021distribution}.
%
Moreover, it is crucial to fully understand how screening algorithms can most effectively and most fairly augment (biased) human decision making in real selection processes. 

